Machine learning reveals features of spinon Fermi surface

With rapid progress in simulation of strongly interacting quantum Hamiltonians, the challenge in characterizing unknown phases becomes a bottleneck for scientific progress. We demonstrate that a Quantum-Classical hybrid approach (QuCl) of mining sampled projective snapshots with interpretable classical machine learning can unveil signatures of seemingly featureless quantum states. The Kitaev-Heisenberg model on a honeycomb lattice under external magnetic field presents an ideal system to test QuCl, where simulations have found an intermediate gapless phase (IGP) sandwiched between known phases, launching a debate over its elusive nature. We use the correlator convolutional neural network, trained on labeled projective snapshots, in conjunction with regularization path analysis to identify signatures of phases. We show that QuCl reproduces known features of established phases. Significantly, we also identify a signature of the IGP in the spin channel perpendicular to the field direction, which we interpret as a signature of Friedel oscillations of gapless spinons forming a Fermi surface. Our predictions can guide future experimental searches for spin liquids.

==> header.tex <==
\AtBeginDocument{
\heavyrulewidth=.08em
\lightrulewidth=.05em
\cmidrulewidth=.03em
\belowrulesep=.65ex
\belowbottomsep=0pt
\aboverulesep=.4ex
\abovetopsep=0pt
\cmidrulesep=\doublerulesep
\cmidrulekern=.5em
\defaultaddspace=.5em
}

\usepackage{float}
\usepackage{comment}
\usepackage{booktabs}
%\usepackage[printwatermark]{xwatermark}
% \usepackage[export]{adjustbox}
% \usepackage[section]{placeins}
%\usepackage[caption=false]{subfig}
\usepackage[percent]{overpic}
\usepackage{microtype}
% \usepackage{widetext}
\usepackage{array}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{physics}
\usepackage{graphicx}
\newtheorem{thm}{Theorem}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{cor}{Corollary}[thm]
\theoremstyle{remark}
\newtheorem*{remark}{Remark}
\theoremstyle{definition}
\newtheorem{eg}{Example}[section]
\newtheorem{definition}{Definition}[section]
\usepackage{bbold}
\numberwithin{thm}{section}
\usepackage{hyperref}
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{tikz}
\usetikzlibrary{arrows.meta, automata, positioning, quotes, shapes}

%% --- citations set up
\bibpunct{[}{]}{,}{n}{}{}
%\bibliographystyle{plainnat}
% \bibliographystyle{apsrev4-1}
\usepackage{hyperref} %boxes hidden, remove hidelinks if boxes are desired.
\hypersetup{colorlinks=true,citecolor=Red,linkcolor=Blue,urlcolor=Blue}
%% ------------------

%% --- manual commands ---
%%my definitions
\newcommand{\xbond}{
	\begin{tikzpicture} [baseline={([yshift=-.5ex]current bounding box.center)}, scale=0.5]
		\begin{scope}[scale=0.3,
			every node/.style={anchor=west,
			draw,
			transform shape,
			minimum width=1cm,
			outer sep=0,
			},
			]
			\node[state, fill=black] (a) {};
			\node[state, fill=black] (b)[above right=1.0cm and 1.732cm of a] {};
			\node[state, densely dotted] (c1)[above=2.0cm of b] {};
			\node[state, densely dotted] (c2)[right=4cm of a] {};
			\node[state, densely dotted] (c3)[left=4cm of b] {};
			\node[state, densely dotted] (c4)[below=2cm of a] {};

			\draw[thick, color=blue] (a) -- (b);
			\draw[dashed] (b) -- (c1);
			\draw[dashed] (b) -- (c2);
			\draw[dashed] (a) -- (c3);
			\draw[dashed] (a) -- (c4);
		\end{scope}
	\end{tikzpicture}
}
\newcommand{\zbond}{
	\begin{tikzpicture} [baseline={([yshift=-.5ex]current bounding box.center)}, scale=0.5]
		\begin{scope}[scale=0.3,
			every node/.style={anchor=west,
			draw,
			transform shape,
			minimum width=1cm,
			outer sep=0,
			},
			]
			\node[state, fill=black] (a) {};
			\node[state, fill=black] (b)[below=2cm of a] {};
			\node[state, densely dotted] (c1)[above right=1cm and 1.732cm of a] {};
			\node[state, densely dotted] (c2)[above left=1cm and 1.732cm of a] {};
			\node[state, densely dotted] (c3)[below right=1cm and 1.732cm of b] {};
			\node[state, densely dotted] (c4)[below left=1cm and 1.732cm of b] {};

			\draw[thick, color=black] (a) -- (b);
			\draw[dashed] (a) -- (c1);
			\draw[dashed] (a) -- (c2);
			\draw[dashed] (b) -- (c3);
			\draw[dashed] (b) -- (c4);
		\end{scope}
	\end{tikzpicture}
}

\newcommand{\bcen}{\begin{center}}
\newcommand{\ecen}{\end{center}}
\newcommand{\btab}{\begin{tabular}}
\newcommand{\etab}{\end{tabular}}
\newcommand{\bdes}{\begin{description}}
\newcommand{\edes}{\end{description}}
\newcommand{\mc}{\multicolumn}
% \newcommand{\ul}{\underline}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\non}{\nonumber}
\newcommand{\etal}{et.~al.\ }
\newcommand{\half}{\frac{1}{2}}
\newcommand{\bary}{\begin{array}}
\newcommand{\eary}{\end{array}}
\newcommand{\benum}{\begin{enumerate}}
\newcommand{\eenum}{\end{enumerate}}
\newcommand{\bitem}{\begin{itemize}}
\newcommand{\eitem}{\end{itemize}}
\newcommand{\cuup}[1]{c_{#1 \uparrow}}
\newcommand{\cdown}[1]{c_{#1 \downarrow}}
\newcommand{\cdup}[1]{c^\dagger_{#1 \uparrow}}
\newcommand{\cddown}[1]{c^\dagger_{#1 \downarrow}}
%
%bold greek characters
%
\newcommand{\al}{\alpha}
\newcommand{\de}{\delta}
\newcommand{\ep}{\epsilon}
\newcommand{\ga}{\gamma}
\newcommand{\lam}{\lambda}
\newcommand{\om}{\omega}
\newcommand{\si}{\sigma}
\newcommand{\dg}{\dagger}
\newcommand{\beps}{\mbox{\boldmath $ \epsilon $}}
\newcommand{\bsig}{\mbox{\boldmath $ \sigma $}}
\newcommand{\bpi}{\mbox{\boldmath $ \pi $}}
\newcommand{\bkap}{\mbox{\boldmath $ \kappa $}}
\newcommand{\bgam}{\mbox{\boldmath $ \gamma $}}
\newcommand{\bphi}{\mbox{\boldmath $ \phi $}}
\newcommand{\balp}{\mbox{\boldmath $ \alpha $}}
\newcommand{\beot}{\mbox{\boldmath $ \eta $}}
\newcommand{\btau}{\mbox{\boldmath $ \tau $}}
\newcommand{\blam}{{\boldsymbol{\lambda}}}
\newcommand{\bomg}{\mbox{\boldmath $ \omega $}}
\newcommand{\bOmg}{\mbox{\boldmath $ \Omega $}}
\newcommand{\bxhi}{\mbox{\boldmath $ \xi $}}
\newcommand{\bmu} {\mbox{\boldmath $ \mu $}}
\newcommand{\bnu} {\mbox{\boldmath $ \nu $}}
\newcommand{\bdelta}{{\boldsymbol{\delta}}}
\newcommand{\bDelta}{{\boldsymbol{\Delta}}}
\newcommand{\bPi}{{\boldsymbol{\Pi}}}
\newcommand{\bpsi}{\mbox{\boldmath $ \psi $}}
\newcommand{\brho}{\mbox{\boldmath $ \rho $}}
\newcommand{\bGam}{{\boldsymbol{\Gamma}}}
\newcommand{\bLam}{\mbox{\boldmath $ \Lambda $}}
\newcommand{\bPhi}{\mbox{\boldmath $ \Phi $}}
\newcommand{\bOne}{{\boldsymbol 1}}
%
%bold latin
%
%\newcommand{\ba} { \mbox{\boldmath $a$}}
\newcommand{\ba} { \bm{a} }
\newcommand{\bb} { \mbox{\boldmath $b$}}
%\newcommand{\bc} { \mbox{\boldmath $c$}}
\newcommand{\bc} { {\mathbf c} }
\newcommand{\bd} { \mbox{\boldmath $d$}}
\newcommand{\be} { \mbox{\boldmath $e$}}
\newcommand{\bff}{ \mbox{\boldmath $f$}}
\newcommand{\bg} { \mbox{\boldmath $g$}}
\newcommand{\bh} { \mbox{\boldmath $h$}}
%\newcommand{\bi} { \mbox{\boldmath $i$}}
\newcommand{\bi}{\bibitem}
\newcommand{\bj} { \mbox{\boldmath $j$}}
\newcommand{\bk} { \bm{k} }
%\newcommand{\bk} { \mbox{\boldmath $k$}}
\newcommand{\bl} { \mbox{\boldmath $l$}} 
\newcommand{\bmm} { \mbox{\boldmath $m$}}
\newcommand{\bn} { \mbox{\boldmath $n$}}
\newcommand{\bo} { \mbox{\boldmath $o$}}
\newcommand{\bp} { \bm{p} }
\newcommand{\bq} { \bm{q} }
%\newcommand{\bq} { \mbox{\boldmath $q$}}
\newcommand{\br} { \boldsymbol{r}}
\newcommand{\bs} { \mbox{\boldmath $s$}}
\newcommand{\bt} {\boldsymbol{t}} 
\newcommand{\bu} { \mbox{\boldmath $u$}}
\newcommand{\bv} { \mbox{\boldmath $v$}}
\newcommand{\bw} { \mbox{\boldmath $w$}}
\newcommand{\bx} { \mbox{\boldmath $x$}}
\newcommand{\by} { \mbox{\boldmath $y$}}
\newcommand{\bz} { \mbox{\boldmath $z$}}

\newcommand{\bA} { \mbox{\boldmath $A$}}
\newcommand{\bB} { \mbox{\boldmath $B$}}
\newcommand{\bC} { \mbox{\boldmath $C$}}
\newcommand{\bD} { \mbox{\boldmath $D$}}
\newcommand{\bE} { \mbox{\boldmath $E$}}
\newcommand{\bF} { \mbox{\boldmath $F$}}
\newcommand{\bG} { \mbox{\boldmath $G$}}
\newcommand{\bH} { \mbox{\boldmath $H$}}
\newcommand{\bI} { \mbox{\boldmath $I$}}
\newcommand{\bJ} { \mbox{\boldmath $J$}}
\newcommand{\bK} {{\textbf{K}}}
\newcommand{\bL} { \mbox{\boldmath $L$}}
\newcommand{\bM} { \mbox{\boldmath $M$}}
\newcommand{\bN} { \mbox{\boldmath $N$}}
\newcommand{\bO} { \mbox{\boldmath $O$}}
\newcommand{\bP} { \mbox{\boldmath $P$}}
\newcommand{\bQ} { \boldsymbol{Q} }
%\newcommand{\bQ} { \mbox{\boldmath $Q$}}
\newcommand{\bR} { {\mathbf R} }
%\newcommand{\bR} { \mbox{\boldmath $R$}}
\newcommand{\bS} { \mbox{\boldmath $S$}}
\newcommand{\bT} { \mbox{\boldmath $T$}}
\newcommand{\bU} { \mbox{\boldmath $U$}}
\newcommand{\bV} { \mbox{\boldmath $V$}}
\newcommand{\bW} { \mbox{\boldmath $W$}}
\newcommand{\bX} { \mbox{\boldmath $X$}}
\newcommand{\bY} { \mbox{\boldmath $Y$}}
\newcommand{\bZ} { \mbox{\boldmath $Z$}}
\newcommand{\bzero} { {\boldsymbol{0}}}
\newcommand{\bfell} {\mbox{\boldmath $ \ell $}}

%
%special math symbols
%
\newcommand{\dou}{\partial}
\newcommand{\leftjb} {[\![}
\newcommand{\rightjb} {]\!]}
\newcommand{\ju}[1]{ \leftjb #1 \rightjb }
\newcommand{\D}[1]{\mbox{d}{#1}} 
% \newcommand{\grad}{\mbox{\boldmath $\nabla$}}
\newcommand{\modulus}[1]{|#1|}
% \renewcommand{\div}[1]{\grad \cdot #1}
% \newcommand{\curl}[1]{\grad \times #1}
\newcommand{\mean}[1]{\langle #1 \rangle}
% \newcommand{\bra}[1]{{\langle #1 |}}
% \newcommand{\ket}[1]{| #1 \rangle}
% \newcommand{\braket}[2]{\langle #1 | #2 \rangle}
\newcommand{\dbdou}[2]{\frac{\dou #1}{\dou #2}}
\newcommand{\dbdsq}[2]{\frac{\dou^2 #1}{\dou #2^2}}
\newcommand{\Pint}[2]{ P \!\!\!\!\!\!\!\int_{#1}^{#2}}
\newcommand{\PARA}[1]{{\noindent {$\bigstar$} {\sc #1}:~}}

%
%abbreviations for equations etc
% 
\newcommand{\eqn}[1] {eqn.~(\ref{#1})}
\newcommand{\prn}[1] {(\ref{#1})}
\newcommand{\sect}[1] {Section~\ref{#1}}
\newcommand{\Sect}[1] {Section~\ref{#1}}
\newcommand{\fig}[1]{fig.~\ref{#1}}
\newcommand{\Fig}[1]{Fig.~\ref{#1}}
\newcommand{\ttau}{\tilde\tau}
\newcommand{\tphi}{\tilde\phi}
\newcommand{\tPhi}{\tilde\Phi}
\newcommand{\tA}{\tilde A}
\newcommand{\tB}{\tilde B}
%\newcommand{\ba}{\bar{a}}
%\newcommand{\bb}{\bar{b}}
%
% Roman Numerals
%
\makeatletter
\newcommand{\rmnum}[1]{\romannumeral #1}
\newcommand{\Rmnum}[1]{\expandafter\@slowromancap\romannumeral #1@}
\makeatother

%
%Other utilities
%
\newcommand{\uncon}[1]{\centerline{\epsfysize=#1 \epsfbox{/usr2/shenoy/styles/construction.eps}}}
\newcommand{\checkup}[1]{{(\tt #1)}\typeout{#1}}
\newcommand{\ttd}[1]{{\color[rgb]{1,0,0}{\bf #1}}}
\newcommand{\ttds}[1]{{\color[rgb]{0,0,1}{\bf #1}}}
\newcommand{\red}[1]{{\color[rgb]{1,0,0}{\protect{#1}}}}
\newcommand{\blue}[1]{{\color[rgb]{0,0,1}{#1}}}
\newcommand{\green}[1]{{\color[rgb]{0.0,0.5,0.0}{#1}}}
\newcommand{\citebyname}[1]{\citeauthor{#1}\cite{#1}}
\newcommand{\signum}[0]{\mathop{\mathrm{sign}}}
\newcommand{\skup}{\ket{s \uparrow}}
\newcommand{\skdn}{\ket{s \downarrow}}
\newcommand{\pkup}{\ket{p \uparrow}}
\newcommand{\pkdn}{\ket{p \downarrow}}
\newcommand{\sbup}{\bra{s \uparrow}}
\newcommand{\sbdn}{\bra{s \downarrow}}
\newcommand{\pbup}{\bra{p \uparrow}}
\newcommand{\pbdn}{\bra{p \downarrow}}

%width of figures
\newcommand{\myfigwidth}{0.4\paperwidth}
\newcommand{\myhalffigwidth}{0.2\paperwidth}

\newcommand{\asc}{a_{sc}}
\newcommand{\as}{a_s}
\newcommand{\Eb}{E_b}
\newcommand{\Ef}{E_F}
\newcommand{\kf}{k_F}
\newcommand{\lambdaT}{{\lambda_T}}
\newcommand{\cF}{{\cal F} }
\newcommand{\ie}{{i.e., } }
\newcommand{\etaT}{{\eta_t}}
\newcommand{\muNI}{{\mu_{NI}}}

%set this to see the name of the labels in the margins
%\newcommand{\mylabel}[1]{\label{#1}{\marginnote{\tiny{\tt #1}}}}
%
%or this for this for doing nothing
\newcommand{\mylabel}[1]{\label{#1}} 

%%
\newcommand{\myonlinecite}[1]{[\onlinecite{#1}]}
%%%%%\newcommand{\mycite}[1]{{\tt[#1]}\cite{#1}}
\newcommand{\mycite}[1]{\cite{#1}}

\newcommand{\sbc}[1]{{\color{red}{#1}}}
\newcommand{\bbc}[1]{{\color{blue}{#1}}}


\definecolor{ForestGreen}{HTML}{668000}
\definecolor{red1}{HTML}{FF4136}
\definecolor{green1}{HTML}{00802b}

\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\up}{\uparrow}
\newcommand{\dn}{\downarrow}

\newcommand{\tcite}{\textcolor{red1}{cite}}
\newcommand{\pdag}{{\phantom\dagger}}
\newcommand{\nirav}[1]{\textcolor{blue}{Nirav: #1}}
\newcommand{\shi}[1]{\textcolor{ForestGreen}{shi: #1}}
\newcommand{\nandini}[1]{\textcolor{red1}{Nandini: #1}}
\newcommand{\todo}[1]{\textcolor{red}{TODO: #1}} % <--- remove before submission
